Measurements of the branching fractions of $\eta_c\to K^+K^-\pi^0$, $K^0_S K^{\pm}\pi^{\mp}$,$2(\pi^+\pi^-\pi^0)$, and $p \bar{p}$

Using data samples collected with the BESIII detector at center-of-mass energies $\sqrt{s} = 4.23, 4.26, 4.36,$ and $4.42$~\rm{GeV}, we measure the branching fractions of $\eta_c\to K^+K^-\pi^0$, $K^0_S K^{\pm}\pi^{\mp}$, $2(\pi^+\pi^-\pi^0)$, and $p \bar{p}$, via the process $e^+e^-\to\pi^+\pi^-h_c$, $h_c\to\gamma\eta_c$. The corresponding results are $(1.15\pm0.12\pm0.10)\%$, $(2.60\pm0.21\pm0.20)\%$, $(15.2\pm1.8\pm1.7)\%$, and $(0.120\pm0.026\pm0.015)\%$, respectively. Here the first uncertainties are statistical, and the second ones systematic. Additionally, the charged track multiplicity of $\eta_c$ decays is measured for the first time.

==> acknowledgement_20180830.tex <==
The BESIII collaboration thanks the staff of BEPCII and the IHEP computing center for their strong support. This work is supported in part by National Key Basic Research Program of China under Contract No. 2015CB856700; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11335008, 11425524, 11625523, 11635010, 11735014; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the CAS Center for Excellence in Particle Physics (CCEPP); Joint Large-Scale Scientific Facility Funds of the NSFC and CAS under Contracts Nos. U1532257, U1532258, U1732263; CAS Key Research Program of Frontier Sciences under Contracts Nos. QYZDJ-SSW-SLH003, QYZDJ-SSW-SLH040; 100 Talents Program of CAS; INPAC and Shanghai Key Laboratory for Particle Physics and Cosmology; German Research Foundation DFG under Contract Nos. Collaborative Research Center CRC 1044, FOR 2359; Istituto Nazionale di Fisica Nucleare, Italy; Koninklijke Nederlandse Akademie van Wetenschappen (KNAW) under Contract No. 530-4CDP03; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Science and Technology fund; The Swedish Research Council; U. S. Department of Energy under Contracts Nos. DE-FG02-05ER41374, DE-SC-0010118, DE-SC-0010504, DE-SC-0012069; University of Groningen (RuG) and the Helmholtzzentrum fuer Schwerionenforschung GmbH (GSI), Darmstadt.


==> author_list_20180830.tex <==
%\author{Author list}
\begin{small}
\begin{center}
M.~Ablikim$^{1}$, M.~N.~Achasov$^{10,d}$, S. ~Ahmed$^{15}$, M.~Albrecht$^{4}$, M.~Alekseev$^{55A,55C}$, A.~Amoroso$^{55A,55C}$, F.~F.~An$^{1}$, Q.~An$^{52,42}$, Y.~Bai$^{41}$, O.~Bakina$^{27}$, R.~Baldini Ferroli$^{23A}$, Y.~Ban$^{35}$, K.~Begzsuren$^{25}$, D.~W.~Bennett$^{22}$, J.~V.~Bennett$^{5}$, N.~Berger$^{26}$, M.~Bertani$^{23A}$, D.~Bettoni$^{24A}$, F.~Bianchi$^{55A,55C}$, J.~Bloms$^{50}$, I.~Boyko$^{27}$, R.~A.~Briere$^{5}$, H.~Cai$^{57}$, X.~Cai$^{1,42}$, A.~Calcaterra$^{23A}$, G.~F.~Cao$^{1,46}$, S.~A.~Cetin$^{45B}$, J.~Chai$^{55C}$, J.~F.~Chang$^{1,42}$, W.~L.~Chang$^{1,46}$, G.~Chelkov$^{27,b,c}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,46}$, J.~C.~Chen$^{1}$, M.~L.~Chen$^{1,42}$, S.~J.~Chen$^{33}$, Y.~B.~Chen$^{1,42}$, W.~Cheng$^{55C}$, G.~Cibinetto$^{24A}$, F.~Cossio$^{55C}$, H.~L.~Dai$^{1,42}$, J.~P.~Dai$^{37,h}$, A.~Dbeyssi$^{15}$, D.~Dedovich$^{27}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{26}$, I.~Denysenko$^{27}$, M.~Destefanis$^{55A,55C}$, F.~De~Mori$^{55A,55C}$, Y.~Ding$^{31}$, C.~Dong$^{34}$, J.~Dong$^{1,42}$, L.~Y.~Dong$^{1,46}$, M.~Y.~Dong$^{1,42,46}$, Z.~L.~Dou$^{33}$, S.~X.~Du$^{60}$, J.~Z.~Fan$^{44}$, J.~Fang$^{1,42}$, S.~S.~Fang$^{1,46}$, Y.~Fang$^{1}$, R.~Farinelli$^{24A,24B}$, L.~Fava$^{55B,55C}$, F.~Feldbauer$^{4}$, G.~Felici$^{23A}$, C.~Q.~Feng$^{52,42}$, M.~Fritsch$^{4}$, C.~D.~Fu$^{1}$, Y.~Fu$^{1}$, Q.~Gao$^{1}$, X.~L.~Gao$^{52,42}$, Y.~Gao$^{44}$, Y.~G.~Gao$^{6}$, Z.~Gao$^{52,42}$, B. ~Garillon$^{26}$, I.~Garzia$^{24A}$, A.~Gilman$^{49}$, K.~Goetzen$^{11}$, L.~Gong$^{34}$, W.~X.~Gong$^{1,42}$, W.~Gradl$^{26}$, M.~Greco$^{55A,55C}$, L.~M.~Gu$^{33}$, M.~H.~Gu$^{1,42}$, Y.~T.~Gu$^{13}$, A.~Q.~Guo$^{1}$, L.~B.~Guo$^{32}$, R.~P.~Guo$^{1,46}$, Y.~P.~Guo$^{26}$, A.~Guskov$^{27}$, S.~Han$^{57}$, X.~Q.~Hao$^{16}$, F.~A.~Harris$^{47}$, K.~L.~He$^{1,46}$, F.~H.~Heinsius$^{4}$, T.~Held$^{4}$, Y.~K.~Heng$^{1,42,46}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,46}$, J.~F.~Hu$^{37,h}$, T.~Hu$^{1,42,46}$, Y.~Hu$^{1}$, G.~S.~Huang$^{52,42}$, J.~S.~Huang$^{16}$, X.~T.~Huang$^{36}$, X.~Z.~Huang$^{33}$, Z.~L.~Huang$^{31}$, T.~Hussain$^{54}$, N.~Hüsken$^{50}$, W.~Ikegami Andersson$^{56}$, W.~Imoehl$^{22}$, M.~Irshad$^{52,42}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{16}$, X.~B.~Ji$^{1,46}$, X.~L.~Ji$^{1,42}$, H.~L.~Jiang$^{36}$, X.~S.~Jiang$^{1,42,46}$, X.~Y.~Jiang$^{34}$, J.~B.~Jiao$^{36}$, Z.~Jiao$^{18}$, D.~P.~Jin$^{1,42,46}$, S.~Jin$^{33}$, Y.~Jin$^{48}$, T.~Johansson$^{56}$, N.~Kalantar-Nayestanaki$^{29}$, X.~S.~Kang$^{34}$, M.~Kavatsyuk$^{29}$, B.~C.~Ke$^{1}$, I.~K.~Keshk$^{4}$, T.~Khan$^{52,42}$, A.~Khoukaz$^{50}$, P. ~Kiese$^{26}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{11}$, L.~Koch$^{28}$, O.~B.~Kolcu$^{45B,f}$, B.~Kopf$^{4}$, M.~Kuemmel$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{56}$, M.~Kurth$^{1}$, W.~K\"uhn$^{28}$, J.~S.~Lange$^{28}$, P. ~Larin$^{15}$, L.~Lavezzi$^{55C}$, H.~Leithoff$^{26}$, C.~Li$^{56}$, Cheng~Li$^{52,42}$, D.~M.~Li$^{60}$, F.~Li$^{1,42}$, F.~Y.~Li$^{35}$, G.~Li$^{1}$, H.~B.~Li$^{1,46}$, H.~J.~Li$^{1,46}$, J.~C.~Li$^{1}$, J.~W.~Li$^{40}$, Ke~Li$^{1}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, P.~L.~Li$^{52,42}$, P.~R.~Li$^{30}$, Q.~Y.~Li$^{36}$, W.~D.~Li$^{1,46}$, W.~G.~Li$^{1}$, X.~L.~Li$^{36}$, X.~N.~Li$^{1,42}$, X.~Q.~Li$^{34}$, X.~H.~Li$^{52,42}$, Z.~B.~Li$^{43}$, H.~Liang$^{52,42}$, Y.~F.~Liang$^{39}$, Y.~T.~Liang$^{28}$, G.~R.~Liao$^{12}$, L.~Z.~Liao$^{1,46}$, J.~Libby$^{21}$, C.~X.~Lin$^{43}$, D.~X.~Lin$^{15}$, B.~Liu$^{37,h}$, B.~J.~Liu$^{1}$, C.~X.~Liu$^{1}$, D.~Liu$^{52,42}$, D.~Y.~Liu$^{37,h}$, F.~H.~Liu$^{38}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, H.~B.~Liu$^{13}$, H.~L~Liu$^{41}$, H.~M.~Liu$^{1,46}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{17}$, J.~B.~Liu$^{52,42}$, J.~Y.~Liu$^{1,46}$, K.~Y.~Liu$^{31}$, Ke~Liu$^{6}$, Q.~Liu$^{46}$, S.~B.~Liu$^{52,42}$, X.~Liu$^{30}$, Y.~B.~Liu$^{34}$, Z.~A.~Liu$^{1,42,46}$, Zhiqing~Liu$^{26}$, Y. ~F.~Long$^{35}$, X.~C.~Lou$^{1,42,46}$, H.~J.~Lu$^{18}$, J.~D.~Lu$^{1,46}$, J.~G.~Lu$^{1,42}$, Y.~Lu$^{1}$, Y.~P.~Lu$^{1,42}$, C.~L.~Luo$^{32}$, M.~X.~Luo$^{59}$, P.~W.~Luo$^{43}$, T.~Luo$^{9,j}$, X.~L.~Luo$^{1,42}$, S.~Lusso$^{55C}$, X.~R.~Lyu$^{46}$, F.~C.~Ma$^{31}$, H.~L.~Ma$^{1}$, L.~L. ~Ma$^{36}$, M.~M.~Ma$^{1,46}$, Q.~M.~Ma$^{1}$, X.~N.~Ma$^{34}$, X.~X.~Ma$^{1,46}$, X.~Y.~Ma$^{1,42}$, Y.~M.~Ma$^{36}$, F.~E.~Maas$^{15}$, M.~Maggiora$^{55A,55C}$, S.~Maldaner$^{26}$, Q.~A.~Malik$^{54}$, A.~Mangoni$^{23B}$, Y.~J.~Mao$^{35}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{55A,55C}$, Z.~X.~Meng$^{48}$, J.~G.~Messchendorp$^{29}$, G.~Mezzadri$^{24A}$, J.~Min$^{1,42}$, T.~J.~Min$^{33}$, R.~E.~Mitchell$^{22}$, X.~H.~Mo$^{1,42,46}$, Y.~J.~Mo$^{6}$, C.~Morales Morales$^{15}$, N.~Yu.~Muchnoi$^{10,d}$, H.~Muramatsu$^{49}$, A.~Mustafa$^{4}$, S.~Nakhoul$^{11,g}$, Y.~Nefedov$^{27}$, F.~Nerling$^{11,g}$, I.~B.~Nikolaev$^{10,d}$, Z.~Ning$^{1,42}$, S.~Nisar$^{8,k}$, S.~L.~Niu$^{1,42}$, S.~L.~Olsen$^{46}$, Q.~Ouyang$^{1,42,46}$, S.~Pacetti$^{23B}$, Y.~Pan$^{52,42}$, M.~Papenbrock$^{56}$, P.~Patteri$^{23A}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{52,42}$, K.~Peters$^{11,g}$, J.~Pettersson$^{56}$, J.~L.~Ping$^{32}$, R.~G.~Ping$^{1,46}$, A.~Pitka$^{4}$, R.~Poling$^{49}$, V.~Prasad$^{52,42}$, M.~Qi$^{33}$, T.~Y.~Qi$^{2}$, S.~Qian$^{1,42}$, C.~F.~Qiao$^{46}$, N.~Qin$^{57}$, X.~S.~Qin$^{4}$, Z.~H.~Qin$^{1,42}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{34}$, K.~H.~Rashid$^{54,i}$, C.~F.~Redmer$^{26}$, M.~Richter$^{4}$, M.~Ripka$^{26}$, A.~Rivetti$^{55C}$, M.~Rolo$^{55C}$, G.~Rong$^{1,46}$, Ch.~Rosner$^{15}$, M.~Rump$^{50}$, A.~Sarantsev$^{27,e}$, M.~Savri\'e$^{24B}$, K.~Schoenning$^{56}$, W.~Shan$^{19}$, X.~Y.~Shan$^{52,42}$, M.~Shao$^{52,42}$, C.~P.~Shen$^{2}$, P.~X.~Shen$^{34}$, X.~Y.~Shen$^{1,46}$, H.~Y.~Sheng$^{1}$, X.~Shi$^{1,42}$, X.~D~Shi$^{52,42}$, J.~J.~Song$^{36}$, Q.~Q.~Song$^{52,42}$, X.~Y.~Song$^{1}$, S.~Sosio$^{55A,55C}$, C.~Sowa$^{4}$, S.~Spataro$^{55A,55C}$, F.~F. ~Sui$^{36}$, G.~X.~Sun$^{1}$, J.~F.~Sun$^{16}$, L.~Sun$^{57}$, S.~S.~Sun$^{1,46}$, X.~H.~Sun$^{1}$, Y.~J.~Sun$^{52,42}$, Y.~K~Sun$^{52,42}$, Y.~Z.~Sun$^{1}$, Z.~J.~Sun$^{1,42}$, Z.~T.~Sun$^{1}$, Y.~T~Tan$^{52,42}$, C.~J.~Tang$^{39}$, G.~Y.~Tang$^{1}$, X.~Tang$^{1}$, B.~Tsednee$^{25}$, I.~Uman$^{45D}$, B.~Wang$^{1}$, B.~L.~Wang$^{46}$, C.~W.~Wang$^{33}$, D.~Y.~Wang$^{35}$, H.~H.~Wang$^{36}$, K.~Wang$^{1,42}$, L.~L.~Wang$^{1}$, L.~S.~Wang$^{1}$, M.~Wang$^{36}$, Meng~Wang$^{1,46}$, P.~Wang$^{1}$, P.~L.~Wang$^{1}$, R.~M.~Wang$^{58}$, W.~P.~Wang$^{52,42}$, X.~Wang$^{35}$, X.~F.~Wang$^{1}$, Y.~Wang$^{52,42}$, Y.~F.~Wang$^{1,42,46}$, Z.~Wang$^{1,42}$, Z.~G.~Wang$^{1,42}$, Z.~Y.~Wang$^{1}$, Zongyuan~Wang$^{1,46}$, T.~Weber$^{4}$, D.~H.~Wei$^{12}$, P.~Weidenkaff$^{26}$, S.~P.~Wen$^{1}$, U.~Wiedner$^{4}$, M.~Wolke$^{56}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,46}$, Z.~Wu$^{1,42}$, L.~Xia$^{52,42}$, Y.~Xia$^{20}$, Y.~J.~Xiao$^{1,46}$, Z.~J.~Xiao$^{32}$, Y.~G.~Xie$^{1,42}$, Y.~H.~Xie$^{6}$, X.~A.~Xiong$^{1,46}$, Q.~L.~Xiu$^{1,42}$, G.~F.~Xu$^{1}$, L.~Xu$^{1}$, Q.~J.~Xu$^{14}$, W.~Xu$^{1,46}$, X.~P.~Xu$^{40}$, F.~Yan$^{53}$, L.~Yan$^{55A,55C}$, W.~B.~Yan$^{52,42}$, W.~C.~Yan$^{2}$, Y.~H.~Yan$^{20}$, H.~J.~Yang$^{37,h}$, H.~X.~Yang$^{1}$, L.~Yang$^{57}$, R.~X.~Yang$^{52,42}$, S.~L.~Yang$^{1,46}$, Y.~H.~Yang$^{33}$, Y.~X.~Yang$^{12}$, Yifan~Yang$^{1,46}$, Z.~Q.~Yang$^{20}$, M.~Ye$^{1,42}$, M.~H.~Ye$^{7}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{43}$, B.~X.~Yu$^{1,42,46}$, C.~X.~Yu$^{34}$, J.~S.~Yu$^{20}$, C.~Z.~Yuan$^{1,46}$, Y.~Yuan$^{1}$, A.~Yuncu$^{45B,a}$, A.~A.~Zafar$^{54}$, Y.~Zeng$^{20}$, B.~X.~Zhang$^{1}$, B.~Y.~Zhang$^{1,42}$, C.~C.~Zhang$^{1}$, D.~H.~Zhang$^{1}$, H.~H.~Zhang$^{43}$, H.~Y.~Zhang$^{1,42}$, J.~Zhang$^{1,46}$, J.~L.~Zhang$^{58}$, J.~Q.~Zhang$^{4}$, J.~W.~Zhang$^{1,42,46}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,46}$, K.~Zhang$^{1,46}$, L.~Zhang$^{44}$, S.~F.~Zhang$^{33}$, T.~J.~Zhang$^{37,h}$, X.~Y.~Zhang$^{36}$, Y.~Zhang$^{52,42}$, Y.~H.~Zhang$^{1,42}$, Y.~T.~Zhang$^{52,42}$, Yang~Zhang$^{1}$, Yao~Zhang$^{1}$, Yu~Zhang$^{46}$, Z.~H.~Zhang$^{6}$, Z.~P.~Zhang$^{52}$, Z.~Y.~Zhang$^{57}$, G.~Zhao$^{1}$, J.~W.~Zhao$^{1,42}$, J.~Y.~Zhao$^{1,46}$, J.~Z.~Zhao$^{1,42}$, Lei~Zhao$^{52,42}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{34}$, Q.~Zhao$^{1}$, S.~J.~Zhao$^{60}$, T.~C.~Zhao$^{1}$, Y.~B.~Zhao$^{1,42}$, Z.~G.~Zhao$^{52,42}$, A.~Zhemchugov$^{27,b}$, B.~Zheng$^{53}$, J.~P.~Zheng$^{1,42}$, Y.~Zheng$^{35}$, Y.~H.~Zheng$^{46}$, B.~Zhong$^{32}$, L.~Zhou$^{1,42}$, Q.~Zhou$^{1,46}$, X.~Zhou$^{57}$, X.~K.~Zhou$^{52,42}$, X.~R.~Zhou$^{52,42}$, Xiaoyu~Zhou$^{20}$, Xu~Zhou$^{20}$, A.~N.~Zhu$^{1,46}$, J.~Zhu$^{34}$, J.~~Zhu$^{43}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,42,46}$, S.~H.~Zhu$^{51}$, X.~L.~Zhu$^{44}$, Y.~C.~Zhu$^{52,42}$, Y.~S.~Zhu$^{1,46}$, Z.~A.~Zhu$^{1,46}$, J.~Zhuang$^{1,42}$, B.~S.~Zou$^{1}$, J.~H.~Zou$^{1}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{8}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{9}$ Fudan University, Shanghai 200443, People's Republic of China\\
$^{10}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{11}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{12}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{13}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{14}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{15}$ Helmholtz Institute Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{16}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{17}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{18}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{19}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{20}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{21}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{22}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{23}$ (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN and University of Perugia, I-06100, Perugia, Italy\\
$^{24}$ (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{25}$ Institute of Physics and Technology, Peace Ave. 54B, Ulaanbaatar 13330, Mongolia\\
$^{26}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{27}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{28}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{29}$ KVI-CART, University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{30}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{31}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{32}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{33}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{34}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{35}$ Peking University, Beijing 100871, People's Republic of China\\
$^{36}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{37}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{38}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{39}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{40}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{41}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{42}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{43}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{44}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{45}$ (A)Ankara University, 06100 Tandogan, Ankara, Turkey; (B)Istanbul Bilgi University, 34060 Eyup, Istanbul, Turkey; (C)Uludag University, 16059 Bursa, Turkey; (D)Near East University, Nicosia, North Cyprus, Mersin 10, Turkey\\
$^{46}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{47}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{48}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{49}$ University of Minnesota, Minneapolis, Minnesota 55455, USA\\
$^{50}$ University of Muenster, Wilhelm-Klemm-Str. 9, 48149 Muenster, Germany\\
$^{51}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{52}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{53}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{54}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{55}$ (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{56}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{57}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{58}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{59}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{60}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at Bogazici University, 34342 Istanbul, Turkey\\
$^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{c}$ Also at the Functional Electronics Laboratory, Tomsk State University, Tomsk, 634050, Russia\\
$^{d}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{e}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{f}$ Also at Istanbul Arel University, 34295 Istanbul, Turkey\\
$^{g}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{h}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{i}$ Also at Government College Women University, Sialkot - 51310. Punjab, Pakistan. \\
$^{j}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{k}$ Also at Harvard University, Department of Physics, Cambridge, MA, 02138, USA\\
}\end{center}
%\vspace{0.4cm}
\end{small}


==> reference.tex <==
\begin{thebibliography}{100}
    \providecommand{\natexlab}[1]{#1}
    \providecommand{\url}[1]{\texttt{#1}}
    \expandafter\ifx\csname urlstyle\endcsname\relax
    \providecommand{\doi}[1]{doi: #1}\else
    \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi
    %===============================================================================
  \bibitem{xyz_states} 
    C.~Z.~Yuan,
    %``The XYZ states revisited,''
    Int.\ J.\ Mod.\ Phys.\ A {\bf 33}, no. 21, 1830018 (2018).
    %doi:10.1142/S0217751X18300181
    %[arXiv:1808.01570 [hep-ex]].
    %%CITATION = doi:10.1142/S0217751X18300181;%%
    %===============================================================================
  \bibitem{getac}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Phys.\ Rev.\ Lett.\ {\bf 108}, 222002 (2012).
    %===============================================================================
  \bibitem{multiplicity}
    K.~Abe {\it et al.} (Belle Collaboration),
    Phys. Rev. Lett. {\bf 89}, 142001 (2002).
    %===============================================================================
  \bibitem{multiplicity_2}
    K.~Abe {\it et al.} (Belle Collaboration),
    Phys. Rev. D. {\bf 70}, 071102 (2004).
    %===============================================================================
  \bibitem{multiplicity_3}
    B.~Aubert {\it et al.} (BABAR Collaboration),
    Phys. Rev. D. {\bf 72}, 031101 (2005).
    %===============================================================================
  \bibitem{guo_aiqiang_etac}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Phys.\ Rev.\ D\ {\bf 86}, 092009 (2012).
    %===============================================================================
  \bibitem{pdg}
    C.~Patrignani {\it et al.} (Particle Data Group),
    Chin.\ Phys.\ C {\bf 40}, 100001 (2016).
    %===============================================================================
  \bibitem{gamma0-}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Phys.\ Rev.\ Lett.\ {\bf 116}, 251802 (2016).
    %===============================================================================
  \bibitem{xyz_luminosities}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Chin.\ Phys.\ C\ {\bf 39}, 093001 (2015).
    %===============================================================================

  \bibitem{guo_yuping_zc}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Phys.\ Rev.\ Lett.\ {\bf 111}, 242001 (2013).
    %===============================================================================
    %  \bibitem{pdg}
    %    M.~Tanabashi {\it et al.} (Particle Data Group),
    %    Phys.\ Rev.\ D\ {\bf98}, 03001 (2018).
    %===============================================================================
  \bibitem{N_psip}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Chin. Phys. C {\bf 37}, 063001 (2013).
    %===============================================================================
  \bibitem{Ablikim:2009aa}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    %``Design and Construction of the BESIII Detector,''
    Nucl.\ Instrum.\ Meth.\ A {\bf 614}, 345 (2010).
    %===============================================================================
  \bibitem{Yu:IPAC2016-TUYA01}
    C.~H.~Yu {\it et al.},
    %``BEPCII Performance and Beam Dynamics Studies on Luminosity,''
    Proceedings of IPAC2016, Busan, Korea, 2016,
  doi:10.18429/JACoW-IPAC2016-TUYA01.	
  %===============================================================================
\bibitem{geant4}
  S.~Agostinelli {\it et al.} (GEANT4 Collaboration),
  %``GEANT4: A Simulation toolkit,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 506}, 250 (2003).
  %===============================================================================
\bibitem{ref:kkmc}
  S.~Jadach, B.~F.~L.~Ward and Z.~Was,
  %``Coherent exclusive exponentiation for precision Monte Carlo calculations,''
  Phys.\ Rev.\ D {\bf 63}, 113009 (2001);
  %``The Precision Monte Carlo event generator K K for two fermion final states in e+ e- collisions,''
  Comput.\ Phys.\ Commun.\  {\bf 130}, 260 (2000).  
  %===============================================================================
\bibitem{ref:evtgen}
  D.~J.~Lange,
  Nucl.\ Instrum.\ Meth.\ A {\bf 462}, 152 (2001);
  R.~G.~Ping,
  Chin. Phys. C {\bf 32}, 599 (2008).
  %===============================================================================

\bibitem{ref:lundcharm}
  J.~C.~Chen, G.~S.~Huang, X.~R.~Qi, D.~H.~Zhang and Y.~S.~Zhu,
  %``Event generator for J / psi and psi (2S) decay,''
  Phys.\ Rev.\ D {\bf 62}, 034003 (2000);
  R.~L.~Yang, R.~G.~Ping and H.~Chen,
  %``Tuning and Validation of the Lundcharm Model with $J/\psi$ Decays,''
  Chin.\ Phys.\ Lett.\  {\bf 31}, 061301 (2014).
  %===============================================================================

\bibitem{photos}
  E.~Richter-Was,
  %``QED bremsstrahlung in semileptonic B and leptonic tau decays,''
  Phys.\ Lett.\ B {\bf 303}, 163 (1993).

  %===============================================================================
\bibitem{vertex}
  M.~Xu {\it et al.} ,
    Chin.\ Phys.\ C {\bf 33} 428 (2009).
    %===============================================================================
  \bibitem{damping_factor_KEDR}
    V.~V.~Anashin {\it et al.},
    Int. J. Mod. Phys. Conf. Ser. 02 188 (2011).
    %\href{http://arXiv.org/abs/1012.1694}
    %{arXiv:1012.1694}.
    %===============================================================================
  \bibitem{R_scan}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Chin. Phys. C 41, 063001 (2017).
    %===============================================================================
  \bibitem{N_Jpsi}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Chin. Phys. C {\bf 36}, 915 (2012).
    %===============================================================================
  \bibitem{kinematic_fit}
    M.~Ablikim {\it et al}. (BESIII Collaboration),
    Phys.\ Rev.\ D\ {\bf 87}, 012002 (2013).
    %===============================================================================
  \bibitem{ks}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Phys.\ Rev.\ D.\ {\bf 91}, 112008 (2015).
    %===============================================================================
    %===============================================================================
  \bibitem{zc_3900}
    M.~Ablikim {\it et al.} (BESIII Collaboration),
    Phys.\ Rev.\ Lett.\ {\bf 119}, 072001 (2017).
    %===============================================================================
  \bibitem{cleo}
    R.~E.~Mitchell {\it et al.} (CLEO Collaboration),
    Phys.\ Rev.\ Lett.\ {\bf 102}, 011801 (2009).
    %===============================================================================
  \bibitem{b2}
    Z.~Sun {\it et al.},
    Phys.\ Rev.\ D.\ {\bf 98}, 094001 (2018).
    %===============================================================================
\end{thebibliography}

